CLAIM: Mitigating Multilingual Object Hallucination in Large Vision-Language Models with Cross-Lingual Attention Intervention

Large Vision-Language Models (LVLMs) have demonstrated impressive multimodal abilities but remain prone to multilingual object hallucination, with a higher likelihood of generating responses inconsistent with the visual input when utilizing queries in non-English languages compared to English. Most existing approaches to address these rely on pretraining or fine-tuning, which are resource-intensive. In this paper, inspired by observing the disparities in cross-modal attention patterns across languages, we propose Cross-Lingual Attention Intervention for Mitigating multilingual object hallucination (CLAIM) in LVLMs, a novel near training-free method by aligning attention patterns. CLAIM first identifies language-specific cross-modal attention heads, then estimates language shift vectors from English to the target language, and finally intervenes in the attention outputs during inference to facilitate cross-lingual visual perception capability alignment. Extensive experiments demonstrate that CLAIM achieves an average improvement of 13.56% (up to 30% in Spanish) on the POPE and 21.75% on the hallucination subsets of the MME benchmark across various languages. Further analysis reveals that multilingual attention divergence is most prominent in intermediate layers, highlighting their critical role in multilingual scenarios.

==> table/main_results.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}

% \begin{table*}[t]\scriptsize
% \centering
% % \setlength{\tabcolsep}{2.5pt}
% \begin{tabular}{cccccccccc}
% \toprule
% Datasets & Setting & Method & \multicolumn{7}{c}{Languages} \\
% \multicolumn{3}{c}{} & En & Zh & De & Fr & Ar & Es & Ru \\
%  &  & Baseline &  & 73.0 & 88.3 & 70.3 & 68.6 & 76.6 & 67.9 \\
%  &  & Compelete Shift &  & 71.3 & 81.3 & 74.7 & 50.4 & 77.2 & 75.2 \\
%  & \multirow{-3}{*}{Random} & Precise Shift & \multirow{-3}{*}{89.8} & {\color[HTML]{FF0000} \cellcolor{lightgreen}87.6(+14.6)}} & 88.3 & {\color[HTML]{FF0000} \cellcolor{lightgreen}77.8(+7.5)}} & {\color[HTML]{00B0F0} 62.6(-6.0)} & {\color[HTML]{FF0000} \cellcolor{lightgreen}80.7(+4.1)}} & {\color[HTML]{FF0000} \cellcolor{lightgreen}86.4(+18.5)}} \\
%  &  & Baseline &  & 70.1 & 86.2 & 75.9 & 69.4 & 76.3 & 60.3 \\
%  &  & Compelete Shift &  & 77.3 & 80.7 & 81.2 & 57.2 & 80.4 & 68.9 \\
%  & \multirow{-3}{*}{Popular} & Precise Shift & \multirow{-3}{*}{86.2} & {\color[HTML]{FF0000} \cellcolor{lightgreen}86.8(+16.7)}} & {\color[HTML]{FF0000} \cellcolor{lightgreen}87.2(+1.0)}} & {\color[HTML]{FF0000} \cellcolor{lightgreen}82.3(+6.4)}} & {\color[HTML]{FF0000} \cellcolor{lightgreen}72.8(+3.4)}} & {\color[HTML]{FF0000} \cellcolor{lightgreen}80.3(+4.0)}} & {\color[HTML]{FF0000} \cellcolor{lightgreen}81.2(+19.9)}} \\
%  &  & Baseline &  & 64.1 & 78.5 & 66.8 & 67.2 & 75.9 & 59.5 \\
%  &  & Compelete Shift &  & 67.6 & 72.6 & 70.7 & 54.9 & 71.0 & 65.6 \\
% \multirow{-9}{*}{POPE-COCO} & \multirow{-3}{*}{Adversarial} & Precise Shift & \multirow{-3}{*}{79.7} & {\color[HTML]{FF0000} \cellcolor{lightgreen}77.7(+13.6)}} & {\color[HTML]{FF0000} \cellcolor{lightgreen}79.2(+0.7)}} & {\color[HTML]{FF0000} \cellcolor{lightgreen}73.5(+6.7)}} & {\color[HTML]{FF0000} \cellcolor{lightgreen}69.1(+1.9)}} & {\color[HTML]{FF0000} \cellcolor{lightgreen}79.2(+3.3)}} & {\color[HTML]{FF0000} \cellcolor{lightgreen}76.2(+16.7)}} \\
%  &  & Baseline &  & 66.5 & 84.3 & 65.6 & 69.9 & 77.3 & 63.9 \\
%  &  & Compelete Shift &  & 66.7 & 75.6 & 69.9 & 50.8 & 71.6 & 71.0 \\
%  & \multirow{-3}{*}{Random} & Precise Shift & \multirow{-3}{*}{87.3} & {\color[HTML]{FF0000} \cellcolor{lightgreen}83.8(+17.3)}} & 84.3 & {\color[HTML]{FF0000} \cellcolor{lightgreen}73.9(+8.3)}} & {\color[HTML]{00B0F0} 62.4(-7.5)} & {\color[HTML]{FF0000} \cellcolor{lightgreen}81.1(+3.8)}} & {\color[HTML]{FF0000} \cellcolor{lightgreen}82.9(+19.0)}} \\
%  &  & Baseline &  & 60.0 & 80.9 & 67.3 & 68.9 & 76.4 & 57.1 \\
%  &  & Compelete Shift &  & 70.2 & 71.8 & 73.9 & 55.0 & 71.4 & 66.7 \\
%  & \multirow{-3}{*}{Popular} & Precise Shift & \multirow{-3}{*}{80.4} & {\color[HTML]{FF0000} \cellcolor{lightgreen}81.5(+21.5)}} & {\color[HTML]{FF0000} 81.2(+0.3)} & {\color[HTML]{FF0000} \cellcolor{lightgreen}80.0(+12.7)}} & {\color[HTML]{00B0F0} 66.1(-2.8)} & {\color[HTML]{FF0000} \cellcolor{lightgreen}80.0(+3.6)}} & {\color[HTML]{FF0000} \cellcolor{lightgreen}77.7(+20.6)}} \\
%  &  & Baseline &  & 56.1 & 71.1 & 59.7 & 66.1 & 73.4 & 56.1 \\
%  &  & Compelete Shift &  & 61.0 & 63.2 & 63.5 & 53.0 & 63.0 & 61.9 \\
% \multirow{-9}{*}{POPE-OKVQA} & \multirow{-3}{*}{Adversarial} & Precise Shift & \multirow{-3}{*}{69.4} & {\color[HTML]{FF0000} \cellcolor{lightgreen}70.9(+14.8)}} & {\color[HTML]{FF0000} 71.2(+0.1)} & {\color[HTML]{FF0000} \cellcolor{lightgreen}67.7(+8.0)}} & {\color[HTML]{00B0F0} 64.3(-1.8)} & {\color[HTML]{FF0000} \cellcolor{lightgreen}76.4(+3.0)}} & {\color[HTML]{FF0000} \cellcolor{lightgreen}70.2(+14.1)}} \\
%  &  & Baseline &  & 68.1 & 84.7 & 66.0 & 65.2 & 77.4 & 63.4 \\
%  &  & Compelete Shift &  & 67.0 & 76.0 & 70.3 & 50.6 & 71.9 & 70.6 \\
%  & \multirow{-3}{*}{Random} & Precise Shift & \multirow{-3}{*}{86.9} & {\color[HTML]{FF0000} \cellcolor{lightgreen}82.9(+14.8)}} & 84.7 & {\color[HTML]{FF0000} \cellcolor{lightgreen}74.5(+8.5)}} & {\color[HTML]{00B0F0} 62.3(-2.9)} & {\color[HTML]{FF0000} \cellcolor{lightgreen}80.0(+2.6)}} & {\color[HTML]{FF0000} \cellcolor{lightgreen}82.4(+19.0)}} \\
%  &  & Baseline &  & 58.4 & 76.4 & 62.1 & 65.5 & 77.4 & 55.9 \\
%  &  & Compelete Shift &  & 65.9 & 66.6 & 67.8 & 55.5 & 66.2 & 62.3 \\
%  & \multirow{-3}{*}{Popular} & Precise Shift & \multirow{-3}{*}{74.5} & {\color[HTML]{FF0000} \cellcolor{lightgreen}76.7(+18.3)}} & {\color[HTML]{FF0000} 76.8(+0.4)} & {\color[HTML]{FF0000} \cellcolor{lightgreen}75.9(+13.8)}} & {\color[HTML]{00B0F0} 64.7(-0.8)} & {\color[HTML]{FF0000} \cellcolor{lightgreen}79.8(+2.4)}} & {\color[HTML]{FF0000} \cellcolor{lightgreen}73.2(+17.3)}} \\
%  &  & Baseline &  & 56.0 & 70.5 & 58.6 & 64.3 & 75.2 & 56.2 \\
%  &  & Compelete Shift &  & 60.1 & 62.3 & 62.5 & 53.8 & 61.9 & 61.5 \\
% \multirow{-9}{*}{POPE-GQA} & \multirow{-3}{*}{Adversarial} & Precise Shift & \multirow{-3}{*}{68.4} & {\color[HTML]{FF0000} \cellcolor{lightgreen}70.5(+14.5)}} & {\color[HTML]{FF0000} 71.2(+0.7)} & {\color[HTML]{FF0000} \cellcolor{lightgreen}67.5(+8.9)}} & {\color[HTML]{FF0000} 66.3(+2.0)} & {\color[HTML]{FF0000} \cellcolor{lightgreen}77.3(+2.1)}} & {\color[HTML]{FF0000} \cellcolor{lightgreen}70.0(+13.8)}} \\
% \multicolumn{2}{c}{} & Baseline &  &  &  &  &  &  &  \\
% \multicolumn{2}{c}{} & Compelete Shift &  &  &  &  &  &  &  \\
% \multicolumn{2}{c}{\multirow{-3}{*}{GQA}} & Precise Shift & \multirow{-3}{*}{} &  &  &  &  &  &  \\
% \multicolumn{2}{c}{} & Baseline &  &  &  &  &  &  &  \\
% \multicolumn{2}{c}{} & Compelete Shift &  &  &  &  &  &  &  \\
% \multicolumn{2}{c}{\multirow{-3}{*}{MME}} & Precise Shift &  &  &  &  &  &  & 
% \end{tabular}
% \end{table*}
\begin{table*}[!ht]
\centering
\small % Smaller font size
\setlength\tabcolsep{3pt} % Baseline value: 6pt
\fontsize{9}{10}\selectfont
% \fontsize{6}{7}\selectfont
\begin{tabular}{lllcccccccccccccc}
\vspace{-5mm}
\toprule
\multirow{2}{*}{\textbf{Dataset}}& \multirow{2}{*}{\textbf{Setup}} & \multirow{2}{*}{\textbf{Method}}& \multicolumn{6}{c}{\textbf{LLaVA-1.5}} & \multicolumn{6}{c}{\textbf{Qwen-VL-Chat}} \\
\cmidrule(lr){4-9} \cmidrule(lr){10-15}
 &  &  & \textbf{En} & \textbf{Zh} & \textbf{Es} & \textbf{Ru} & \textbf{Pt} & \textbf{Bg} & \textbf{En}&\textbf{Zh} & \textbf{Es} & \textbf{Ru} & \textbf{Hi} & \textbf{De}\\
\midrule
\multirow{9}{*}{POPE-COCO} & \multirow{3}{*}{Random} & \textit{Baseline} & {88.50} & 81.00 & 63.03 & 72.33 & 78.97 & 72.23 & 86.63 &84.57&68.13&76.83&56.97&77.53 \\
 &  & \textit{VCD} & -& 81.47 & 67.40 & 73.33 & 78.07 & 72.47 &  -& 84.70&72.17&75.37&48.37&78.27 \\
&  & \textit{Ours} & -& \cellcolor{lightgreen}86.50 & \cellcolor{lightgreen}87.33 & \cellcolor{lightgreen}87.50 & \cellcolor{lightgreen}85.40 & \cellcolor{lightgreen}80.50 &  -&\cellcolor{lightgreen}88.03&\cellcolor{lightgreen}86.93&\cellcolor{lightgreen}82.60&\cellcolor{lightgreen}67.57&\cellcolor{lightgreen}88.07  \\
 % \addlinespace 
  \cmidrule(lr){3-15} 
  & \multirow{3}{*}{Popular} & \textit{Baseline} & {87.43} & 83.07 & 62.93 & 69.20 &	82.03&	71.17	& 85.67&83.40&68.03&75.73&62.20&77.20	\\
 &  & \textit{VCD} & -&83.20  & 67.20 &	70.17	& 80.10	&69.47&-	&82.70&72.70&74.20&57.40&76.70& \\
&  & \textit{Ours} & -&\cellcolor{lightgreen}88.00 & \cellcolor{lightgreen}87.53 & \cellcolor{lightgreen}84.03 & \cellcolor{lightgreen}86.13 & \cellcolor{lightgreen}80.07 & - & \cellcolor{lightgreen}85.47&\cellcolor{lightgreen}85.90&\cellcolor{lightgreen}80.63&\cellcolor{lightgreen}69.23&\cellcolor{lightgreen}86.43  \\
  \cmidrule(lr){3-15} 
  & \multirow{3}{*}{Adversarial} & \textit{Baseline} & {85.20}& 73.40 & 62.87 & 66.07	&73.70&	65.93	&83.90&	80.87&67.53&72.80&63.10&75.90 \\
 &  & \textit{VCD} & -& 74.27	& 67.30	& 66.47	&73.63	&66.33	&	-&79.40&71.97&70.83&54.73&75.03& \\
&  & \textit{Ours} & -& \cellcolor{lightgreen}77.67 & \cellcolor{lightgreen}83.27 & \cellcolor{lightgreen}79.43 & \cellcolor{lightgreen}79.67 & \cellcolor{lightgreen}74.57 &  -&\cellcolor{lightgreen}82.33&\cellcolor{lightgreen}80.70&\cellcolor{lightgreen}77.53&\cellcolor{lightgreen}69.70&\cellcolor{lightgreen}81.50  \\
 \midrule
 
 \multirow{9}{*}{POPE-OKVQA} & \multirow{3}{*}{Random} & \textit{Baseline} & {91.00} & 76.13 & 63.40 & 70.30 &	75.03&	69.23	&88.47&85.10&67.70&74.63&59.53&75.17	 \\
 &  & \textit{VCD} & -&77.93 & 68.17	& 72.17	& 75.67	&70.33	&-&	84.30&72.23&73.67&49.07&75.33\\
&  & \textit{Ours} & -&\cellcolor{lightgreen}86.80 & \cellcolor{lightgreen}85.97 & \cellcolor{lightgreen}85.63 & \cellcolor{lightgreen}83.87 & \cellcolor{lightgreen}80.63 & - &\cellcolor{lightgreen}88.13 &\cellcolor{lightgreen}86.03&\cellcolor{lightgreen}83.47&\cellcolor{lightgreen}68.83&\cellcolor{lightgreen}86.13  \\
  \cmidrule(lr){3-15} 
  & \multirow{3}{*}{Popular} & \textit{Baseline} & {86.97}	& 74.50 &	63.27&	69.40&	77.03&	67.73&	88.70&85.60&67.90&75.43&58.87&75.27	 \\
 &  & \textit{VCD} & -&77.57 & 67.10 &68.40 &	77.03	&68.20	&-	&84.17	&71.57&73.30&52.40&75.63 \\
&  & \textit{Ours} & -&\cellcolor{lightgreen}85.00 & \cellcolor{lightgreen}83.40 & \cellcolor{lightgreen}81.87 & \cellcolor{lightgreen}84.27 & \cellcolor{lightgreen}77.97 & - & \cellcolor{lightgreen}88.10&\cellcolor{lightgreen}85.70&\cellcolor{lightgreen}83.90&\cellcolor{lightgreen}68.50&\cellcolor{lightgreen}86.03  \\
  \cmidrule(lr){3-15} 
  & \multirow{3}{*}{Adversarial} & \textit{Baseline} & {79.57}&	64.40&	62.37&	63.93&	67.97&	63.03&	82.40&79.97&66.80&72.50&60.17&72.30	 \\
 &  & \textit{VCD} & -&68.97 &	65.17&	63.90 &	68.67&	64.07 &	 - &	78.77&69.00&69.63&50.80&71.90	 \\
&  & \textit{Ours} & -&\cellcolor{lightgreen}77.70 & \cellcolor{lightgreen}75.40 & \cellcolor{lightgreen}76.17 & \cellcolor{lightgreen}75.67 & \cellcolor{lightgreen}71.97 &  -&\cellcolor{lightgreen}81.10&\cellcolor{lightgreen}77.20&\cellcolor{lightgreen}78.73&\cellcolor{lightgreen}67.73&\cellcolor{lightgreen}78.87  \\
 \midrule
 \multirow{9}{*}{POPE-GQA} & \multirow{3}{*}{Random} & \textit{Baseline} & 89.47	&77.03	&63.83	& 70.23&	74.87&	68.07&87.23 &82.53 &73.03 &74.00 &\cellcolor{lightgreen}65.10 &74.30	\\
 &  & \textit{VCD} & -&78.00	&68.33	& 71.47 &	73.63&	70.20& -& 83.63&76.10 &73.43 &55.50 &80.20\\
&  & \textit{Ours} & -&\cellcolor{lightgreen}84.27 & \cellcolor{lightgreen}85.13 & \cellcolor{lightgreen}83.57 & \cellcolor{lightgreen}82.53  & \cellcolor{lightgreen}82.67 &- &\cellcolor{lightgreen}85.17 &\cellcolor{lightgreen}79.93 &\cellcolor{lightgreen}81.90&62.03 &\cellcolor{lightgreen}80.40 &  \\
  \cmidrule(lr){3-15} 
  & \multirow{3}{*}{Popular} & \textit{Baseline} & 83.90& 	69.60& 64.03& 	64.53& 	71.53& 	63.40&85.80 &81.90 &72.17 &75.07 &59.20 &70.40 	 \\
 &  & \textit{VCD} & -&73.60	& 67.50& 	65.23 &71.87& 	66.20 &- &82.20 &73.73 &74.17 &54.70 &76.87 	\\
&  & \textit{Ours} & -&\cellcolor{lightgreen}81.57 & \cellcolor{lightgreen}78.50 & \cellcolor{lightgreen}77.93 & \cellcolor{lightgreen}79.60  & \cellcolor{lightgreen}80.57 &- & \cellcolor{lightgreen}84.43&\cellcolor{lightgreen}80.60 &\cellcolor{lightgreen}82.60 &\cellcolor{lightgreen}61.30&\cellcolor{lightgreen}78.07  \\
  \cmidrule(lr){3-15} 
  & \multirow{3}{*}{Adversarial} & \textit{Baseline} & 81.17& 	63.17& 	63.30	&64.10	& 67.90	& 62.10	& 82.63&78.97&69.73 &73.07 &61.73 & 71.63 & \\
 &  & \textit{VCD} & -&67.33	& 66.97	& 63.87	&67.83 & 	63.37 & -& 79.57&73.47 & 71.83&54.97 &76.17 \\
&  & \textit{Ours} & -&\cellcolor{lightgreen}77.57 & \cellcolor{lightgreen}75.93 & \cellcolor{lightgreen}76.27 & \cellcolor{lightgreen}75.23  & \cellcolor{lightgreen}76.47 & -&\cellcolor{lightgreen}79.97 &\cellcolor{lightgreen}76.77 &\cellcolor{lightgreen}79.53 &\cellcolor{lightgreen}62.47 &\cellcolor{lightgreen}77.63  \\
\midrule
\multirow{15}{*}{MME}&\multirow{3}{*}{Existence}&\textit{Baseline}&190.0&175.0&130.0&145.0&155.0&125.0&185.0&190.0&135.0&140.0&106.7&195.0\\
& &\textit{VCD}&-&180.0&130.0&145.0&150.0&128.3&-&185.0&155.0&155.0&78.30&195.0\\
& &\textit{Ours}&-&\cellcolor{lightgreen}195.0&\cellcolor{lightgreen}175.0&\cellcolor{lightgreen}185.0&\cellcolor{lightgreen}175.0&\cellcolor{lightgreen}180.0&-&\cellcolor{lightgreen}190.0&\cellcolor{lightgreen}155.0&\cellcolor{lightgreen}185.0&\cellcolor{lightgreen}128.3&\cellcolor{lightgreen}195.0\\
&\multirow{3}{*}{Count}&\textit{Baseline}&155.0&70.00&55.00&58.30&80.00&85.00&150.0&130.0&143.3&113.3&60.00&136.7\\
& &\textit{VCD}&-&73.30&73.30&53.30&61.70&105.0&-&140.0&131.7&100.0&80.00&128.3\\
& &\textit{Ours}&-&\cellcolor{lightgreen}125.0&\cellcolor{lightgreen}130.0&\cellcolor{lightgreen}110.0&\cellcolor{lightgreen}130.0&\cellcolor{lightgreen}135.0&-&\cellcolor{lightgreen}148.3&\cellcolor{lightgreen}153.3&\cellcolor{lightgreen}120.0&\cellcolor{lightgreen}111.7&\cellcolor{lightgreen}137.0\\
&\multirow{3}{*}{Color}&\textit{Baseline}&165.0&80.00&135.0&75.00&110.0&80.00&180.0&170.0&150.0&153.3&\cellcolor{lightgreen}103.3&165.0\\
& &\textit{VCD}&-&95.00&145.0&85.00&130.0&88.30&-&150.0&165.0&146.7&93.30&160.0\\
& &\textit{Ours}&-&\cellcolor{lightgreen}120.0&\cellcolor{lightgreen}155.0&\cellcolor{lightgreen}125.0&\cellcolor{lightgreen}150.0&\cellcolor{lightgreen}108.3&-&\cellcolor{lightgreen}170.0&\cellcolor{lightgreen}165.0&\cellcolor{lightgreen}158.3&90.00&\cellcolor{lightgreen}165.0\\
&\multirow{3}{*}{Position}&\textit{Baseline}&118.3&53.30&63.30&55.00&50.00&46.70&131.7&63.30&\cellcolor{lightgreen}120.0&93.30&45.00&105.0\\
& &\textit{VCD}&-&48.30&\cellcolor{lightgreen}93.00&60.00&51.70&56.70&-&\cellcolor{lightgreen}78.30&101.7&101.7&43.30&93.30\\
& &\textit{Ours}&-&\cellcolor{lightgreen}66.70&78.30&\cellcolor{lightgreen}85.00&\cellcolor{lightgreen}86.70&\cellcolor{lightgreen}58.30&-&63.30&116.7&\cellcolor{lightgreen}103.3&\cellcolor{lightgreen}55.00&\cellcolor{lightgreen}106.0\\
&\multirow{3}{*}{Total Scores}&\textit{Baseline}&628.3&378.3&383.3&333.3&395.0&336.7&646.7&553.3&548.3&500.0&315.0&601.7\\
& &\textit{VCD}&-&396.7&441.3&343.3&393.3&378.3&-&553.3&556.7&503.3&295.0&576.7\\
& &\textit{Ours}&-&\cellcolor{lightgreen}506.7&\cellcolor{lightgreen}538.3&\cellcolor{lightgreen}505.0&\cellcolor{lightgreen}541.7&\cellcolor{lightgreen}481.7&-&\cellcolor{lightgreen}571.7&\cellcolor{lightgreen}590.0&\cellcolor{lightgreen}566.6&\cellcolor{lightgreen}385.0&\cellcolor{lightgreen}603.0\\
\bottomrule
\end{tabular}
\caption{Main results on POPE and hallucination subset of MME. \colorbox{lightgreen}{Green} means the best perfomance.}

\label{tab:POPE}
\end{table*}
